Efficient Generation of One-Factorizations through Hill Climbing

It is well known that for every even integer $n$, the complete graph $K_{n}$ has a one-factorization, namely a proper edge coloring with $n-1$ colors. Unfortunately, not much is known about the possible structure of large one-factorizations. Also, at present we have only woefully few explicit constructions of one-factorizations. Specifically, we know essentially nothing about the {\em typical} properties of one-factorizations for large $n$. Suppose that $\cal C_{\rm n}$ is a graph whose vertex set includes the set of all order-$n$ one-factorizations and that $\Psi: V(\cal C_{\rm n})\to \mathbb R$ takes its minimum precisely at the one-factorizations. Given $\cal C_{\rm n}$ and $\Psi$, we can generate one-factorizations via hill climbing. Namely, by taking a walk on $\cal C_{\rm n}$ that tends to go from a vertex to a neighbor of smaller $\Psi$. For over 30 years, hill-climbing has been essentially the only method for generating many large one-factorizations. However, the validity of such methods was supported so far only by numerical evidence. Here, we present for the first time hill-climbing algorithms that provably generate an order-$n$ one-factorization in $\text{polynomial}(n)$ steps regardless of the starting state, while all vertex degrees in the underlying graph are appropriately bounded. We also raise many questions and conjectures regarding hill-climbing methods and concerning the possible and typical structure of one-factorizations.

==> Before_Fix.tex <==
\begin{tikzpicture}[ every arrow/.append style={dash,thick}, node distance =2 cm and 2cm ]
    \node[shape=circle,draw=black] (1) at (0,0) {$v_1$};
    \node[shape=circle,draw=black, label={\small $\text{missing green}$}] (2) at (.5,1.8) {$v_2$};
    \node[shape=circle,draw=black] (3) at (1,0) {$v_3$};
    \path (1) edge[line width=0.3mm, red] (2);
    \path (2) edge[line width=0.3mm,red] (3); 
    \node[shape=circle,draw=black] (4) at (3,0) {$u_1$};
    \node[shape=circle,draw=black, label={\small $\text{missing blue}$}] (5) at (3.5,1.8) {$u_2$};
    \node[shape=circle,draw=black] (6) at (4,0) {$u_3$};
    \path (4) edge[line width=0.3mm,red] (5);
    \path (5) edge[line width=0.3mm,red] (6); 
\end{tikzpicture}

==> Vee.tex <==
\begin{tikzpicture}[ every arrow/.append style={dash,thick}, node distance =2 cm and 2cm ]
    \node[shape=circle,draw=black] (1) at (5,0) {x};
    \node[shape=circle,draw=black] (2) at (5.5,1.8) {a};
    \node[shape=circle,draw=black] (3) at (6,0) {};
    \path (1) edge[red] (2);
    \path (2) edge[red] (3); 
\end{tikzpicture}



